O1 Replication Journey -- Part 2: Surpassing O1-preview through Simple Distillation, Big Progress or Bitter Lesson?

This paper presents a critical examination of current approaches to replicating OpenAI's O1 model capabilities, with particular focus on the widespread but often undisclosed use of knowledge distillation techniques. While our previous work explored the fundamental technical path to O1 replication, this study reveals how simple distillation from O1's API, combined with supervised fine-tuning, can achieve superior performance on complex mathematical reasoning tasks. Through extensive experiments, we show that a base model fine-tuned on simply tens of thousands of samples O1-distilled long-thought chains outperforms O1-preview on the American Invitational Mathematics Examination (AIME) with minimal technical complexity. Moreover, our investigation extends beyond mathematical reasoning to explore the generalization capabilities of O1-distilled models across diverse tasks: hallucination, safety and open-domain QA. Notably, despite training only on mathematical problem-solving data, our models demonstrated strong generalization to open-ended QA tasks and became significantly less susceptible to sycophancy after fine-tuning. We deliberately make this finding public to promote transparency in AI research and to challenge the current trend of obscured technical claims in the field. Our work includes: (1) A detailed technical exposition of the distillation process and its effectiveness, (2) A comprehensive benchmark framework for evaluating and categorizing O1 replication attempts based on their technical transparency and reproducibility, (3) A critical discussion of the limitations and potential risks of over-relying on distillation approaches, our analysis culminates in a crucial bitter lesson: while the pursuit of more capable AI systems is important, the development of researchers grounded in first-principles thinking is paramount.

==> learning-method-comparison.tex <==


\begin{table*}[!t]
    \centering
    \setlength{\tabcolsep}{6pt}
    {
    \fontsize{10}{13}\selectfont % 设置字体大小为10pt，行距为13pt
    \renewcommand\arraystretch{1.2}
    \resizebox{\linewidth}{!}{
        \begin{tabular}[l]{lll}
        \toprule
        \textbf{Characteristic} & \textbf{Shortcut Learning} & \textbf{Journey Learning} \\ \midrule
        \multirow{1}{*}{\textbf{Learning Objective}} & Quickly achieve specific tasks or metrics & Comprehensive deep understanding, continuous improvement \\ 
        \multirow{1}{*}{\textbf{Learning Depth}} & Surface features and simple correlations & Deep causal relationships and underlying principles \\ 
        \multirow{1}{*}{\textbf{Adaptability}} & Limited to specific tasks or data distributions & Broadly adaptable to different contexts and tasks \\ 
        \multirow{1}{*}{\textbf{Reasoning Ability}} & Limited, struggles with complex reasoning & Powerful, demonstrates human-like reasoning \\ 
        \multirow{1}{*}{\textbf{Self-Improvement}} & Lacks self-correction mechanisms & Continuous self-assessment and improvement \\ 
        \multirow{1}{*}{\textbf{Learning Process}} & Static, one-time training & Dynamic, continuous learning and adaptation \\ 
        \multirow{1}{*}{\textbf{Generalization}} & Limited, easily affected by data distribution changes & Strong, can handle new situations \\ 
        \multirow{1}{*}{\textbf{Innovation Capacity}} & Limited, struggles to solve new problems & High, can generate innovative solutions \\ 
        \multirow{1}{*}{\textbf{Data Dependency}} & Highly dependent on large training datasets & More focused on quality and learning strategies \\ 
        \multirow{1}{*}{\textbf{Computational Efficiency}} & Often requires significant computational resources & Potentially more efficient, focusing on strategy over scale \\ 
        \multirow{1}{*}{\textbf{Interpretability}} & Poor, often seen as a "black box" & Better, can track internal reasoning processes \\ 
        \multirow{1}{*}{\textbf{Ethical Considerations}} & May unintentionally amplify data biases & Easier to implement ethical constraints and adjustments \\ 
        \multirow{1}{*}{\textbf{Security}} & Vulnerable to adversarial attacks & More robust, able to identify potential threats \\ 
        \multirow{1}{*}{\textbf{Long-term Value}} & Quick results in specific tasks & Paves the way for AGI development \\ 
        \multirow{1}{*}{\textbf{Human Analogy}} & Exam-oriented education, crash courses & Comprehensive education, lifelong learning \\ 
        \bottomrule
        \end{tabular}
    }
    \caption{Comparison between Shortcut Learning and Journey Learning.}
    \label{tab:comparison}
    }
\end{table*}



==> o1-math-graph.tex <==
% Define tcolorbox style


\definecolor{wkblue}{rgb}{0.2, 0.3, 0.6}
\definecolor{meta-color}{rgb}{0.5, 0.5, 0.5}

\begin{tcolorbox}[colback=wkblue!10!white, colframe=wkblue!100!blue, left=2mm, right=2mm, title=\small\centering\textcolor{black}{The Thought Structure of OpenAI o1 in Mathematical Reasoning}]
\begin{small}

\# Problem: Solving the equation $p(1/x) = x^2$ 

\vspace{1.6mm}

\#\# Step 1: Define $q(x) = p(1/x) - x^2$

\begin{itemize}
    \item Analyze the roots of $q(x)$:
    \begin{itemize}
        \item \textbf{Therefore}: $q(k) = 0$ for $k = \pm 1, \pm 2, \dots, \pm n$
    \end{itemize}
    \item Let me consider: Construct $s(x) = x^{2n}q(x)$
    \begin{itemize}
        \item Analyze the properties of $s(x)$:
        \begin{itemize}
            \item \textbf{Therefore}: $s(x)$ is a polynomial
        \end{itemize}
        \item \textbf{Alternatively}: Consider $s(x) = x^{2n}p(1/x) - x^{2n+2}$
        \begin{itemize}
            \item \textbf{Let me explain}: Expand the expression for \( p(1/x) \).
        \end{itemize}
        \item Factorize $s(x) = m(x)h(x)$
        \begin{itemize}
            \item Define $m(x) = \prod(x^2 - k^2)$
            \item Hypothesize the form of $h(x)$:
            \begin{itemize}
                \item \textbf{Consider}: $h(x)$ must be a quadratic polynomial
                \item \textbf{Try}: $h(x) = -x^2 + bx + c$
                
                \item \textbf{Wait}: We need to determine the values of $b$ and $c$
                \item \textbf{Let me compute}: Determine the coefficients of \( h(x) \)      
            \end{itemize}
        \end{itemize}
    \end{itemize}
\end{itemize}

\vspace{1.6mm}

\#\# Step 2: Alternatively, construct $t(x) = x^{2n}p(1/x) = p^*(x)$

\begin{itemize}
    \item Analyze the properties of $p^*(x)$:
    \begin{itemize}
        \item \textbf{Therefore}: $p^*(x)$ is the reciprocal polynomial of $p(x)$
    \end{itemize}
    \item Consider $s(x) = t(x) - x^{2n+2}$
    \begin{itemize}
        \item \textbf{Thus}: $s(x) = p*(x) - x^(2n+2)$
    \end{itemize}
    \item Let me consider the coefficients of $( p^*(x) )$
    \begin{itemize}
        \item Analyze the constant term: \( p^*(0) = 1 \)
        \item Analyze the coefficient of the \( x^{2n} \) term: \( a_0 = c \)
    \end{itemize}
\end{itemize}

\vspace{1.6mm}

\#\# Step 3: \textbf{Let me compute}: Expand \( m(x)h(x) \)

\begin{itemize}
    \item Analyze the higher-order terms: $-x^{2n+2} + cx^{2n}$
    \item Compare with \( s(x) \): \( -x^{2n+2} + [\text{lower degree terms}] \)
    \begin{itemize}
        \item \textbf{Thus}: Confirm \( h(x) = -x^2 + c \)
    \end{itemize}
\end{itemize}


\vspace{1.6mm}

\#\# Step 4: \textbf{Wait}: Let us reconsider the value of $m(x)$ at $x = 0$

\begin{itemize}
    \item Compute: $m(0) = (-1)^n (n!)^2$
    \item Consider: \( s(0) = m(0)h(0) = 1 \)
    \item Therefore: \( c = \frac{(-1)^n}{(n!)^2} \)
    \begin{itemize}
        \item Verify: This is consistent with the previous result
    \end{itemize}
\end{itemize}

\vspace{1.6mm}

\#\# Step 5: \textbf{So}: Solve $h(x) = 0$

\begin{itemize}
    \item $-x^2 + c = 0$
    \item $x^2 = c = \frac{1}{(n!)^2}$
    \item \textbf{Therefore}:Additional solutions are $x = \pm 1/n!$
    \item \textbf{Wait}: We need to consider the case when \( n \) is even
    \begin{itemize}
        \item When \( n \) is even: \( c > 0 \)
        \item \textbf{Verify}: This ensures that the solutions are real
    \end{itemize}
\end{itemize}

\end{small}
\end{tcolorbox}


% \setlistdepth{9}

% \definecolor{wkblue}{rgb}{0.2, 0.3, 0.6}
% \definecolor{meta-color}{rgb}{0.5, 0.5, 0.5}

% \begin{tcolorbox}[colback=wkblue!10!white, colframe=wkblue!100!blue, left=2mm, right=2mm, title=\small\textcolor{black}{The Thought Structure of OpenAI o1 in Mathematical Reasoning}]
% \begin{small}

% \# Solving the equation $p(1/x) = x^2$ \hfill\textcolor{meta-color}{\# We're trying to solve a polynomial equation.}

% \vspace{1.6mm}

% \#\# Step 1: Define $q(x) = p(1/x) - x^2$ \hfill\textcolor{meta-color}{\# Define a new function to simplify the problem.}

% \begin{itemize}
%     \item Analyze the roots of $q(x)$: \hfill\textcolor{meta-color}{\# We need to find where $q(x)$ equals zero.}
%     \begin{itemize}
%         \item \textbf{Therefore}: $q(k) = 0$ for $k = \pm 1, \pm 2, \dots, \pm n$ \hfill\textcolor{meta-color}{\# The roots of $q(x)$ are $k = \pm 1, \pm 2, \dots, \pm n$.}
%     \end{itemize}
%     \item Let me consider: Construct $s(x) = x^{2n}q(x)$ \hfill\textcolor{meta-color}{\# create a new polynomial $s(x)$.}
%     \begin{itemize}
%         \item Analyze the properties of $s(x)$: \hfill\textcolor{meta-color}{\# Investigate how $s(x)$ behaves as a polynomial.}
%         \begin{itemize}
%             \item \textbf{Therefore}: $s(x)$ is a polynomial \hfill\textcolor{meta-color}{\# Confirm that $s(x)$ is a polynomial.}
%         \end{itemize}
%         \item \textbf{Alternatively}: Consider $s(x) = x^{2n}p(1/x) - x^{2n+2}$ \hfill\textcolor{meta-color}{\# Express $s(x)$ in terms of $p(1/x)$ for further analysis.}
%         \begin{itemize}
%             \item \textbf{Let me explain}: Expand the expression for \( p(1/x) \). \hfill\textcolor{meta-color}{\# We need to expand $p(1/x)$ to see its full form.}
%         \end{itemize}
%         \item Factorize $s(x) = m(x)h(x)$ \hfill\textcolor{meta-color}{\# Break $s(x)$ into simpler factors.}
%         \begin{itemize}
%             \item Define $m(x) = \prod(x^2 - k^2)$ \hfill\textcolor{meta-color}{\# Define $m(x)$ based on the product of squared terms.}
%             \item Hypothesize the form of $h(x)$: \hfill\textcolor{meta-color}{\# Now, let's guess the form of $h(x)$.}
%             \begin{itemize}
%                 \item \textbf{Consider}: $h(x)$ must be a quadratic polynomial \hfill\textcolor{meta-color}{\# Assume $h(x)$ is a quadratic polynomial.}
%                 \item \textbf{Try}: $h(x) = -x^2 + bx + c$ \hfill\textcolor{meta-color}{\# Propose a specific form for $h(x)$.}
                
%                 \item \textbf{Wait}: We need to determine the values of $b$ and $c$ \hfill\textcolor{meta-color}{\# Pause to calculate the coefficients $b$ and $c$.}
%                 \item \textbf{Let me compute}: Determine the coefficients of \( h(x) \) \hfill\textcolor{meta-color}{\# Perform the actual calculation of $b$ and $c$.}
%             \end{itemize}
%         \end{itemize}
%     \end{itemize}
% \end{itemize}

% \vspace{1.6mm}

% \#\# Step 2: Alternatively, construct $t(x) = x^{2n}p(1/x) = p^*(x)$

% \begin{itemize}
%     \item Analyze the properties of $p^*(x)$: \hfill\textcolor{meta-color}{\# Investigate the characteristics of $p^*(x)$.}
%     \begin{itemize}
%         \item \textbf{Therefore}: $p^*(x)$ is the reciprocal polynomial of $p(x)$ \hfill\textcolor{meta-color}{\# Confirm that $p^*(x)$ is a reciprocal polynomial.}
%     \end{itemize}
%     \item Consider $s(x) = t(x) - x^{2n+2}$ \hfill\textcolor{meta-color}{\# Define $s(x)$ as the difference between $t(x)$ and a higher degree term.}
%     \begin{itemize}
%         \item \textbf{Thus}: $s(x) = p*(x) - x^(2n+2)$ \hfill\textcolor{meta-color}{\# Confirm the structure of $s(x)$.}
%     \end{itemize}
%     \item Let me consider the coefficients of $( p^*(x) )$ \hfill\textcolor{meta-color}{\# Focus on analyzing the specific coefficients of $p^*(x)$.}
%     \begin{itemize}
%         \item Analyze the constant term: \( p^*(0) = 1 \) \hfill\textcolor{meta-color}{\# Note that the constant term of $p^*(x)$ is 1.}
%         \item Analyze the coefficient of the \( x^{2n} \) term: \( a_0 = c \) \hfill\textcolor{meta-color}{\# Identify the coefficient of the $x^{2n}$ term.}
%     \end{itemize}
% \end{itemize}

% \vspace{1.6mm}

% \#\# Step 3: \textbf{Let me compute}: Expand \( m(x)h(x) \) \hfill\textcolor{meta-color}{\# Now, expand the product $m(x)h(x)$ to examine its form.}

% \begin{itemize}
%     \item Analyze the higher-order terms: $-x^{2n+2} + cx^{2n}$ \hfill\textcolor{meta-color}{\# Focus on the highest degree terms in the expansion.}
%     \item Compare with \( s(x) \): \( -x^{2n+2} + [\text{lower degree terms}] \) \hfill\textcolor{meta-color}{\# Match these terms with those in $s(x)$.}
%     \begin{itemize}
%         \item \textbf{Thus}: Confirm \( h(x) = -x^2 + c \) \hfill\textcolor{meta-color}{\# Conclude that $h(x)$ has the expected form.}
%     \end{itemize}
% \end{itemize}


% \vspace{1.6mm}

% \#\# Step 4: \textbf{Wait}: Let us reconsider the value of $m(x)$ at $x = 0$ \hfill\textcolor{meta-color}{\# Pause to recalculate $m(x)$ when $x = 0$.}

% \begin{itemize}
%     \item Compute: $m(0) = (-1)^n (n!)^2$ \hfill\textcolor{meta-color}{\# Calculate $m(0)$ using a factorial expression.}
%     \item Consider: \( s(0) = m(0)h(0) = 1 \) \hfill\textcolor{meta-color}{\# Now, use $m(0)$ and $h(0)$ to find $s(0)$.}
%     \item Therefore: \( c = \frac{(-1)^n}{(n!)^2} \) \hfill\textcolor{meta-color}{\# Derive $c$ from the previous computations.}
%     \begin{itemize}
%         \item Verify: This is consistent with the previous result \hfill\textcolor{meta-color}{\# Ensure this result matches earlier findings.}
%     \end{itemize}
% \end{itemize}

% \vspace{1.6mm}

% \#\# Step 5: \textbf{So}: Solve $h(x) = 0$ \# Solve the equation $h(x) = 0$.

% \begin{itemize}
%     \item $-x^2 + c = 0$ \hfill\textcolor{meta-color}{\# Set the quadratic expression equal to zero.}
%     \item $x^2 = c = \frac{1}{(n!)^2}$ \hfill\textcolor{meta-color}{\# Solve for $x^2$.}
%     \item \textbf{Therefore}:Additional solutions are $x = \pm 1/n!$ \hfill\textcolor{meta-color}{\# The solutions for $x$ are $\pm 1/n!$.}
%     \item \textbf{Wait}: We need to consider the case when \( n \) is even \hfill\textcolor{meta-color}{\# Pause to reflect on the case where $n$ is even.}
%     \begin{itemize}
%         \item When \( n \) is even: \( c > 0 \) \hfill\textcolor{meta-color}{\# When $n$ is even, $c$ is positive.}
%         \item \textbf{Verify}: This ensures that the solutions are real \hfill\textcolor{meta-color}{\# This confirms that the solutions are real numbers.}
%     \end{itemize}
% \end{itemize}

% \end{small}
% \end{tcolorbox}



==> our-case1.tex <==
% \definecolor{wkblue}{rgb}{0.2, 0.3, 0.6}
% \definecolor{meta-color}{rgb}{0.5, 0.5, 0.5}

% \begin{tcolorbox}[colback=wkblue!10!white, colframe=wkblue!100!blue, left=2mm, right=2mm, title=\small\centering\textcolor{black}{The Thought Structure of Our Thought in Mathematical Reasoning}]
% \begin{small}

% \# Problem: Find the remainder when $$f(x)=x^{10}+5x^9-8x^8+7x^7-x^6-12x^5+4x^4-8x^3+12x^2-5x-5$$ is divided by $x^2-1$ without using long division.

% \vspace{1.6mm}

% \#\# Apply the Remainder Theorem

% \begin{itemize}
%     \item \textbf{We want to} find the remainder when $f(x)$ is divided by $x^2 - 1$.
%     \item Using the Remainder Theorem. 
%     \begin{itemize}
%         \item Substitute \( x = 1 \) and \( x = -1 \) into \( f(x) \) to find the remainders at those points.
%         \item \textbf{Let me compute} \( f(1) \):
%         \begin{align*}
%         f(1) &= 1^{10} + 5(1)^9 - 8(1)^8 + 7(1)^7 - 1^6 - 12(1)^5 + 4(1)^4 - 8(1)^3 + 12(1)^2 - 5(1) - 5 \\
%               &= 1 + 5 - 8 + 7 - 1 - 12 + 4 - 8 + 12 - 5 - 5 \\
%               &= -10
%         \end{align*}
%         \item \textbf{Similarly}, calculate \( f(-1) \):
%         \begin{align*}
%         f(-1) &= (-1)^{10} + 5(-1)^9 - 8(-1)^8 + 7(-1)^7 - (-1)^6 - 12(-1)^5 + 4(-1)^4 - 8(-1)^3 \\
%         &\quad\quad + 12(-1)^2 - 5(-1) - 5 \\
%               &= 1 - 5 - 8 - 7 - 1 + 12 + 4 + 8 + 12 + 5 - 5 \\
%               &= 16
%         \end{align*}
%         \item \textbf{Therefore}: The remainder when dividing by \( x - 1 \) is \(-10\), and for \( x + 1 \) it is \( 16 \).
%     \end{itemize}
% \end{itemize}

% \vspace{1.6mm}

% \#\# Deriving the remainder \( r(x) = ax + b \)

% \begin{itemize}
%     \item \textbf{Since} \( x^2 - 1 = (x - 1)(x + 1) \), the remainder must be of the form \( ax + b \).
%     \item We now solve for \( a \) and \( b \) using the remainders from \textbf{Step 1}.
%     \begin{itemize}
%         \item Set up the system of equations:
%         \begin{align*}
%         a(1) + b &= -10 \quad \text{(from \( f(1) = -10 \))} \\
%         a(-1) + b &= 16 \quad \text{(from \( f(-1) = 16 \))}
%         \end{align*}
%         \item \textbf{Let me compute}: Add the equations to find \( b \):
%         \begin{align*}
%         a + b &= -10 \\
%         -a + b &= 16 \\
%         \text{Adding the equations}: 2b &= 6 \quad \Rightarrow \quad b = 3
%         \end{align*}
%         \item Now substitute \( b = 3 \) into \( a + b = -10 \):
%         \begin{align*}
%         a + 3 &= -10 \quad \Rightarrow \quad a = -13
%         \end{align*}
%     \end{itemize}
% \end{itemize}

% \vspace{1.6mm}

% \#\# \textbf{Thus}: The remainder when \( f(x) \) is divided by \( x^2 - 1 \) is \( -13x + 3 \).
% \vspace{1.6mm}

% \#\# Final result: \( r(x) = \boxed{-13x + 3} \)



% \end{small}
% \end{tcolorbox}


\definecolor{wkblue}{rgb}{0.2, 0.3, 0.6}
\definecolor{meta-color}{rgb}{0.5, 0.5, 0.5}
\definecolor{pinkcolor}{rgb}{1.0, 0.75, 0.8}  % 柔和的粉色

\begin{tcolorbox}[colback=pinkcolor!10!white, colframe=pinkcolor!100!red, left=2mm, right=2mm, title=\small\centering\textcolor{black}{Case 2: Solution to The Remainder Problem}]
\begin{small}
\# Problem: Find the remainder when $$f(x)=x^{10}+5x^9-8x^8+7x^7-x^6-12x^5+4x^4-8x^3+12x^2-5x-5$$ is divided by $x^2-1$ without using long division.
\vspace{1.6mm}

\# Our Proposed Model Response:

\vspace{1.6mm}
First, we need to find the remainder when \( f(x) \) is divided by \( x^2 - 1 \). 
To do this, we can use the Remainder Theorem, which states that if we divide a polynomial \( f(x) \) by \( x - a \), the remainder is \( f(a) \).

Now, let's apply this to our problem. We need to find the remainder when \( f(x) \) is divided by \( x^2 - 1 \). 
This suggests that we should substitute \( x = 1 \) and \( x = -1 \) into \( f(x) \) to find the remainders.

Let's start with \( x = 1 \). Substituting this into \( f(x) \), we get:

\[
f(1) = 1^{10} + 5(1)^9 - 8(1)^8 + 7(1)^7 - (1)^6 - 12(1)^5 + 4(1)^4
- 8(1)^3 + 12(1)^2 - 5(1) - 5
\]

Calculating this step-by-step:

\[
1^{10} = 1, \quad 5(1)^9 = 5, \quad -8(1)^8 = -8, \quad 7(1)^7 = 7, \quad -(1)^6 = -1, \quad -12(1)^5 = -12, \quad 4(1)^4 = 4, ...
\]

Adding these values together, we find:

\[
f(1) = 1 + 5 - 8 + 7 - 1 - 12 + 4 - 8 + 12 - 5 - 5 = -10
\]

So, the remainder when \( f(x) \) is divided by \( x - 1 \) is \( -10 \).

Now, \textcolor{red}{let's try} \( x = -1 \):

\[
f(-1) = (-1)^{10} + 5(-1)^9 - 8(-1)^8 + 7(-1)^7 - (-1)^6 - 12(-1)^5 + 4(-1)^4 - 8(-1)^3 + 12(-1)^2 - 5(-1) - 5
\]

Calculating each term:

\[
(-1)^{10} = 1, \quad 5(-1)^9 = -5, \quad -8(-1)^8 = -8, \quad 7(-1)^7 = -7, \quad -(-1)^6 = -1, \quad -12(-1)^5 = 12, ...
\]

Adding these values, we get:

\[
f(-1) = 1 - 5 - 8 - 7 - 1 + 12 + 4 + 8 + 12 + 5 - 5 = 16
\]

Therefore, the remainder when \( f(x) \) is divided by \( x + 1 \) is \( 16 \).

\textcolor{red}{Let's pause and consider what we know so far}. We have found the remainders when \( f(x) \) is divided by \( x - 1 \) and \( x + 1 \). 
Now, we need to use these results to determine the remainder when \( f(x) \) is divided by \( x^2 - 1 \).

Since \( x^2 - 1 \) can be factored as \( (x - 1)(x + 1) \), the remainder when \( f(x) \) is divided by \( x^2 - 1 \) should be a linear expression \( ax + b \).

\textcolor{red}{Let's express} \( f(x) \) as: \(
f(x) = (x^2 - 1) q(x) + ax + b
\), where \( q(x) \) is the quotient.

\textcolor{red}{At this point}, we know:

\begin{itemize}
    \item When \( f(x) \) is divided by \( x - 1 \), the remainder is \( -10 \).
    \item When \( f(x) \) is divided by \( x + 1 \), the remainder is \( 16 \).
\end{itemize}

Let's use these to find \( a \) and \( b \).

First, consider the Remainder Theorem:

\begin{itemize}
    \item Substituting \( x = 1 \), we have: 
    \quad \(
    f(1) = a(1) + b = -10
    \)
    \item Substituting \( x = -1 \):
    \quad \quad \quad \quad \(
    f(-1) = a(-1) + b = 16
    \)
\end{itemize}

Let's solve these equations simultaneously:

From the first equation:
\quad\quad\quad\quad\quad\quad\quad \(
a + b = -10
\)

From the second equation:
\quad\quad\quad\quad\quad\quad \(
-a + b = 16
\)

Adding these equations gives:
\quad\quad\quad\quad\quad \(
2b = 6 \quad \Rightarrow \quad b = 3
\)

Substituting back into \( a + b = -10 \):
\quad\quad \(
a + 3 = -10 \quad \Rightarrow \quad a = -13
\)

So, the remainder when \( f(x) \) is divided by \( x^2 - 1 \) is:

\[
-13x + 3
\]

To summarize, the remainder is \( \boxed{-13x + 3} \).

\end{small}
\end{tcolorbox}


==> our-case2.tex <==
% \definecolor{wkblue}{rgb}{0.2, 0.3, 0.6}
% \definecolor{meta-color}{rgb}{0.5, 0.5, 0.5}

% \begin{tcolorbox}[colback=wkblue!10!white, colframe=wkblue!100!blue, left=2mm, right=2mm, title=\small\centering\textcolor{black}{The Thought Structure of Our Thought in Mathematical Reasoning}]
% \begin{small}

% \# Problem: Find all possible values of 
% \[
% \frac{1}{1 + \omega} + \frac{1}{1 + \omega^2}
% \]
% where \( \omega^3 = 1 \).

% \vspace{1.6mm}

% \#\# Understanding the cube roots of unity

% \begin{itemize}
%     \item The cube roots of unity are the solutions to \( \omega^3 = 1 \), which gives us three possible values: 
%     \[
%     \omega = 1, \quad \omega = \frac{-1 + i\sqrt{3}}{2}, \quad \omega = \frac{-1 - i\sqrt{3}}{2}.
%     \]
% \end{itemize}

% \vspace{1.6mm}

% \#\# Calculate the expression for \( \omega = 1 \)

% \begin{itemize}
%     \item Substituting \( \omega = 1 \) into the expression:
%     \[
%     \frac{1}{1 + 1} + \frac{1}{1 + 1} = \frac{1}{2} + \frac{1}{2} = 1.
%     \]
% \end{itemize}

% \vspace{1.6mm}

% \#\# Calculate the expression for \( \omega = \frac{-1 + i\sqrt{3}}{2} \)

% \begin{itemize}
%     \item Substituting \( \omega = \frac{-1 + i\sqrt{3}}{2} \) into the expression:
%     \[
%     \frac{1}{1 + \frac{-1 + i\sqrt{3}}{2}} + \frac{1}{1 + \frac{-1 - i\sqrt{3}}{2}}.
%     \]
%     Simplifying both terms:
%     \[
%     1 + \frac{-1 + i\sqrt{3}}{2} = \frac{1 + i\sqrt{3}}{2}, \quad 1 + \frac{-1 - i\sqrt{3}}{2} = \frac{1 - i\sqrt{3}}{2}.
%     \]
%     \item This gives:
%     \[
%     \frac{1}{\frac{1 + i\sqrt{3}}{2}} + \frac{1}{\frac{1 - i\sqrt{3}}{2}} = \frac{2}{1 + i\sqrt{3}} + \frac{2}{1 - i\sqrt{3}}.
%     \]
%     Simplifying each term using conjugates:
%     \[
%     \frac{2}{1 + i\sqrt{3}} = \frac{1 - i\sqrt{3}}{2}, \quad \frac{2}{1 - i\sqrt{3}} = \frac{1 + i\sqrt{3}}{2}.
%     \]
%     Adding these gives:
%     \[
%     \frac{1 - i\sqrt{3}}{2} + \frac{1 + i\sqrt{3}}{2} = 1.
%     \]
% \end{itemize}

% \vspace{1.6mm}

% \#\# Calculate the expression for \( \omega = \frac{-1 - i\sqrt{3}}{2} \)

% \begin{itemize}
%     \item This case is symmetrical to the previous one. Substituting \( \omega = \frac{-1 - i\sqrt{3}}{2} \) into the expression yields the same steps and result:
%     \[
%     \frac{1 - i\sqrt{3}}{2} + \frac{1 + i\sqrt{3}}{2} = 1.
%     \]
% \end{itemize}

% \vspace{1.6mm}

% \#\# \textbf{Thus}: For all possible values of \( \omega \), the expression simplifies to \( \boxed{1} \).


% \end{small}
% \end{tcolorbox}


% \definecolor{wkblue}{rgb}{0.2, 0.3, 0.6}
% \definecolor{meta-color}{rgb}{0.5, 0.5, 0.5}

% \begin{tcolorbox}[colback=wkblue!10!white, colframe=wkblue!100!blue, left=2mm, right=2mm, title=\small\centering\textcolor{black}{Solution to Polynomial Product Problem}]
% \begin{small}

% \# Problem: The product of \( (3t^2 + 5t + a)(4t^2 + bt - 2) \) is given as \( 12t^4 + 26t^3 - 8t^2 - 16t + 6 \). What is \( a + b \)?

% \vspace{1.6mm}

% \#\# Expand the product

% \begin{itemize}
%     \item \textbf{First, We need to} expand the product \( (3t^2 + 5t + a)(4t^2 + bt - 2) \).
%     \item When we do this, we should carefully multiply each term carefully:
%     \begin{align*}
%         (3t^2)(4t^2) &= 12t^4, \\
%         (3t^2)(bt) &= 3bt^3, \\
%         (3t^2)(-2) &= -6t^2, \\
%         (5t)(4t^2) &= 20t^3, \\
%         (5t)(bt) &= 5bt^2, \\
%         (5t)(-2) &= -10t, \\
%         (a)(4t^2) &= 4at^2, \\
%         (a)(bt) &= abt, \\
%         (a)(-2) &= -2a.
%     \end{align*}
% \end{itemize}

% \vspace{1.6mm}

% \#\# Combine like terms

% \begin{itemize}
%     \item \textbf{Now, let's} combine like terms:
%     \begin{align*}
%         t^4 \text{ term}: &\quad 12t^4, \\
%         t^3 \text{ terms}: &\quad (3bt^3 + 20t^3) = (3b + 20)t^3, \\
%         t^2 \text{ terms}: &\quad (-6t^2 + 5bt^2 + 4at^2) = (-6 + 5b + 4a)t^2, \\
%         t \text{ terms}: &\quad (-10t + abt) = (-10 + ab)t, \\
%         \text{Constant term}: &\quad -2a.
%     \end{align*}
% \end{itemize}

% \vspace{1.6mm}

% \#\# Compare coefficients with the given expression

% \begin{itemize}
%     \item The expanded expression needs to match the given polynomial \( 12t^4 + 26t^3 - 8t^2 - 16t + 6 \).
%     \item \textbf{Let's} equate the coefficients of like terms:
%     \begin{itemize}
%         \item For the \( t^4 \) term: \( 12 = 12 \), which checks.
%         \item For the \( t^3 \) term: \( 26 = 3b + 20 \), solving gives \( b = 2 \).
%         \item For the \( t^2 \) term: \( -8 = -6 + 5b + 4a \), substituting \( b = 2 \) gives:
%         \[
%         -8 = -6 + 10 + 4a \quad \Rightarrow \quad -8 = 4 + 4a \quad \Rightarrow \quad 4a = -12 \quad \Rightarrow \quad a = -3.
%         \]
%         \item For the \( t \) term: \( -16 = -10 + ab \), substituting \( a = -3 \) and \( b = 2 \), we get:
%         \[
%         -16 = -10 - 6, \quad \text{which checks}.
%         \]
%         \item For the constant term: \( 6 = -2a \), substituting \( a = -3 \), we get:
%         \[
%         6 = 6, \quad \text{which checks}.
%         \]
%     \end{itemize}
% \end{itemize}

% \vspace{1.6mm}

% \#\# Correcting the mistake

% \begin{itemize}
%     \item \textbf{Wait a second}: There seems to be a mistake in the constant term calculation. Let's correct it:
%     \item The correct equation should be \( 6 = -2a \), solving this gives:
%     \[
%     a = -3.
%     \]
% \end{itemize}

% \vspace{1.6mm}

% \#\# With \( a = -3 \) and \( b = 2 \), we find:
%     \[
%     a + b = -3 + 2 = \boxed{-1}.
%     \]


% \end{small}
% \end{tcolorbox}


\definecolor{wkblue}{rgb}{0.2, 0.3, 0.6}
\definecolor{meta-color}{rgb}{0.5, 0.5, 0.5}
\definecolor{pinkcolor}{rgb}{1.0, 0.75, 0.8}  % 柔和的粉色


\begin{tcolorbox}[colback=pinkcolor!10!white, colframe=pinkcolor!100!red, left=2mm, right=2mm, title=\small\centering\textcolor{black}{Case 1: Solution to Algebra Problem with Polynomial Multiplication}]

\begin{small}

\# Problem: The product of $3t^2+5t+a$ and $4t^2+bt-2$ is $12t^4+26t^3-8t^2-16t+6$. What is $a+b$?

\vspace{1.6mm}

\# Our Proposed Model Response:

\vspace{1.6mm}

First, we need to expand the product \((3t^2 + 5t + a)(4t^2 + bt - 2)\).

When we do this, we should \textcolor{red}{carefully} multiply each term:

\begin{itemize}
    \item The product of \(3t^2\) and \(4t^2\) gives us \(12t^4\).
    \item The product of \(3t^2\) and \(bt\) gives us \(3bt^3\).
    \item The product of \(3t^2\) and \(-2\) gives us \(-6t^2\).
    \item The product of \(5t\) and \(4t^2\) gives us \(20t^3\).
    \item The product of \(5t\) and \(bt\) gives us \(5bt^2\).
    \item The product of \(5t\) and \(-2\) gives us \(-10t\).
    \item The product of \(a\) and \(4t^2\) gives us \(4at^2\).
    \item The product of \(a\) and \(bt\) gives us \(abt\).
    \item The product of \(a\) and \(-2\) gives us \(-2a\).
\end{itemize}

Now, let's combine like terms:

\begin{itemize}
    \item The \(t^4\) term is \(12t^4\), so we have \(12t^4\).
    \item The \(t^3\) terms are \(3bt^3\) and \(20t^3\), which combine to \((3b + 20)t^3\).
    \item The \(t^2\) terms are \(-6t^2\), \(5bt^2\), and \(4at^2\), which combine to \((-6 + 5b + 4a)t^2\).
    \item The \(t\) terms are \(-10t\) and \(abt\), which combine to \((-10 + ab)t\).
    \item The constant term is \(-2a\).
\end{itemize}

\textcolor{red}{Let's pause} and consider what we know so far. We need this expanded expression to match the given polynomial \(12t^4 + 26t^3 - 8t^2 - 16t + 6\).

Now, let's equate the coefficients of like terms:

\begin{itemize}
    \item For the \(t^4\) term, we have \(12 = 12\), which checks.
    \item For the \(t^3\) term, we get \(26 = 3b + 20\). Solving gives \(b = 2\).
    \item For the \(t^2\) term, we have \(-8 = -6 + 5b + 4a\). Substituting \(b = 2\), we get \(-8 = -6 + 10 + 4a\), which simplifies to \(4a = -14\) and \(a = -3.5\).
    \item For the \(t\) term, we have \(-16 = -10 + ab\). Substituting \(a = -3.5\) and \(b = 2\), we get \(-16 = -10 - 7\), which checks.
    \item For the constant term, we have \(6 = -2a\). Substituting \(a = -3.5\), we get \(6 = 7\), \textcolor{red}{which doesn't check}.
\end{itemize}

\textcolor{red}{Wait a second}, let's check our calculations again. The constant term calculation should have been \(6 = -2a\), which gives \(a = -3\). \textcolor{red}{Let's go back and correct that.}

With \(a = -3\) and \(b = 2\), we find \(a + b = -3 + 2 = -1\).

So, the correct value of \(a + b\) is \(\boxed{-1}\).

\end{small}
\end{tcolorbox}


==> our-case3.tex <==
\definecolor{wkblue}{rgb}{0.2, 0.3, 0.6}
\definecolor{meta-color}{rgb}{0.5, 0.5, 0.5}
\definecolor{pinkcolor}{rgb}{1.0, 0.75, 0.8}  % 柔和的粉色

\begin{tcolorbox}[colback=pinkcolor!10!white, colframe=pinkcolor!100!red, left=2mm, right=2mm, title=\small\centering\textcolor{black}{Case 3: Solution to Number Theory Problem with Multiples of 30}]
\begin{small}

\# Problem: What is the least positive integer multiple of 30 that can be written with only the digits 0 and 2?

\vspace{1.6mm}

\# Our Proposed Model Response:

\vspace{1.6mm}

We need to find the least positive integer multiple of 30 that can be formed using only the digits 0 and 2.

To start, we know that a number is divisible by 30 if it is divisible by both 10 and 3. Let's address each condition separately.

First, let's consider the divisibility by 10. A number is divisible by 10 if it ends in 0. So, we need to ensure that our number ends in 0.

Now, let's focus on the divisibility by 3. A number is divisible by 3 if the sum of its digits is divisible by 3. Let's calculate the sum of the digits using only the digits 0 and 2.

The digits available are 0 and 2. The sum of these digits is \(0 + 2 = 2\).

\textcolor{red}{At this point}, we have a sum of 2, which is not divisible by 3. Let's pause and consider what this means. Since 2 is not divisible by 3, the number formed using only the digits 0 and 2 will not be divisible by 3 either.

\textcolor{red}{Let's rethink this}. Perhaps we're missing something. Maybe we can adjust the digits to make the sum divisible by 3.

\textcolor{red}{Let's reconsider} the sum of the digits. If we use both digits, 0 and 2, we can form different combinations to see if the sum becomes divisible by 3.

Let's try different combinations:
\begin{itemize}
    \item Using only 0, the sum is 0.
    \item Using only 2, the sum is 2.
    \item Using both, the sum can be \(0 + 2 = 2\) or \(2 + 0 = 2\).
\end{itemize}

Clearly, the sum of 2 is not divisible by 3. Let's try combining the digits differently.

\textcolor{red}{Wait, maybe I'm missing something again}. Let's reconsider the combinations. If we use both digits, we can form larger numbers by arranging them differently. Let's try:
\begin{itemize}
    \item 20: Sum is \(2 + 0 = 2\).
    \item 22: Sum is \(2 + 2 = 4\).
    \item 202: Sum is \(2 + 0 + 2 = 4\).
\end{itemize}

Still, the sums of 2 and 4 are not divisible by 3. Let's try something different.

Let's try using larger numbers formed by rearranging the digits:
\begin{itemize}
    \item 200: Sum is \(2 + 0 + 0 = 2\).
    \item 220: Sum is \(2 + 2 + 0 = 4\).
    \item 2020: Sum is \(2 + 0 + 2 + 0 = 4\).
\end{itemize}

Still, the sums of 2 and 4 are not divisible by 3. Let's try one more approach.

Let's consider using more digits:
\begin{itemize}
    \item 2220: Sum is \(2 + 2 + 2 + 0 = 6\).
\end{itemize}

Now, the sum of 6 is divisible by 3. Let's pause and consider what this means. Since 2220 ends in 0, it is divisible by 10. Therefore, 2220 is divisible by both 10 and 3, making it divisible by 30.

So, the least positive integer multiple of 30 that can be formed using only the digits 0 and 2 is \( \boxed{2220} \).

\end{small}
\end{tcolorbox}


==> table/case-study-code.tex <==
% \definecolor{wkblue}{rgb}{0.2, 0.3, 0.6}
% \definecolor{meta-color}{rgb}{0.5, 0.5, 0.5}

% \begin{tcolorbox}[colback=wkblue!10!white, colframe=wkblue!100!blue, left=2mm, right=2mm, title=\small\centering\textcolor{black}{The Thought Structure of Our Thought in Mathematical Reasoning}]
% \begin{small}

% \# Problem: Find the remainder when $$f(x)=x^{10}+5x^9-8x^8+7x^7-x^6-12x^5+4x^4-8x^3+12x^2-5x-5$$ is divided by $x^2-1$ without using long division.

% \vspace{1.6mm}

% \#\# Apply the Remainder Theorem

% \begin{itemize}
%     \item \textbf{We want to} find the remainder when $f(x)$ is divided by $x^2 - 1$.
%     \item Using the Remainder Theorem. 
%     \begin{itemize}
%         \item Substitute \( x = 1 \) and \( x = -1 \) into \( f(x) \) to find the remainders at those points.
%         \item \textbf{Let me compute} \( f(1) \):
%         \begin{align*}
%         f(1) &= 1^{10} + 5(1)^9 - 8(1)^8 + 7(1)^7 - 1^6 - 12(1)^5 + 4(1)^4 - 8(1)^3 + 12(1)^2 - 5(1) - 5 \\
%               &= 1 + 5 - 8 + 7 - 1 - 12 + 4 - 8 + 12 - 5 - 5 \\
%               &= -10
%         \end{align*}
%         \item \textbf{Similarly}, calculate \( f(-1) \):
%         \begin{align*}
%         f(-1) &= (-1)^{10} + 5(-1)^9 - 8(-1)^8 + 7(-1)^7 - (-1)^6 - 12(-1)^5 + 4(-1)^4 - 8(-1)^3 \\
%         &\quad\quad + 12(-1)^2 - 5(-1) - 5 \\
%               &= 1 - 5 - 8 - 7 - 1 + 12 + 4 + 8 + 12 + 5 - 5 \\
%               &= 16
%         \end{align*}
%         \item \textbf{Therefore}: The remainder when dividing by \( x - 1 \) is \(-10\), and for \( x + 1 \) it is \( 16 \).
%     \end{itemize}
% \end{itemize}

% \vspace{1.6mm}

% \#\# Deriving the remainder \( r(x) = ax + b \)

% \begin{itemize}
%     \item \textbf{Since} \( x^2 - 1 = (x - 1)(x + 1) \), the remainder must be of the form \( ax + b \).
%     \item We now solve for \( a \) and \( b \) using the remainders from \textbf{Step 1}.
%     \begin{itemize}
%         \item Set up the system of equations:
%         \begin{align*}
%         a(1) + b &= -10 \quad \text{(from \( f(1) = -10 \))} \\
%         a(-1) + b &= 16 \quad \text{(from \( f(-1) = 16 \))}
%         \end{align*}
%         \item \textbf{Let me compute}: Add the equations to find \( b \):
%         \begin{align*}
%         a + b &= -10 \\
%         -a + b &= 16 \\
%         \text{Adding the equations}: 2b &= 6 \quad \Rightarrow \quad b = 3
%         \end{align*}
%         \item Now substitute \( b = 3 \) into \( a + b = -10 \):
%         \begin{align*}
%         a + 3 &= -10 \quad \Rightarrow \quad a = -13
%         \end{align*}
%     \end{itemize}
% \end{itemize}

% \vspace{1.6mm}

% \#\# \textbf{Thus}: The remainder when \( f(x) \) is divided by \( x^2 - 1 \) is \( -13x + 3 \).
% \vspace{1.6mm}

% \#\# Final result: \( r(x) = \boxed{-13x + 3} \)



% \end{small}
% \end{tcolorbox}


% \definecolor{wkblue}{rgb}{0.2, 0.3, 0.6}
% \definecolor{meta-color}{rgb}{0.5, 0.5, 0.5}
% \definecolor{pinkcolor}{rgb}{1.0, 0.75, 0.8}  % soft pink

% \begin{tcolorbox}[
%     colback=pinkcolor!10!white,
%     colframe=pinkcolor!100!red,
%     left=2mm,
%     right=2mm,
%     title=\small\centering\textcolor{black}{Understanding await asyncio.sleep() Issues},
%     breakable=true,
%     % break at={\pagebreak},         % 只在明确的分页点处分页
% ]
% \begin{tiny}

% \# Problem: Why in python await asyncio.sleep() is such?

% \vspace{1.6mm}

% \# Our Proposed Model Response:

% \vspace{1.6mm}

% \textbf{Understanding asyncio.sleep()}

% First, it's important to understand what \texttt{asyncio.sleep()} does:
% \begin{itemize}
%     \item \texttt{asyncio.sleep()} is a coroutine function that suspends the execution of the coroutine for a given number of seconds.
%     \item During the sleep, other tasks can run, making it useful for simulating delays without blocking the entire program.
%     \item It's commonly used in asynchronous programming to introduce delays or to simulate IO-bound operations.
% \end{itemize}

% \textbf{Common Reasons Why await asyncio.sleep() Might Seem Stuck}

% 1. \textbf{Event Loop Not Running}
%    \begin{itemize}
%    \item \textit{Explanation:} The asyncio event loop is responsible for managing and scheduling coroutines. If the event loop isn't running, the coroutines won't execute, and \texttt{await asyncio.sleep()} will appear stuck.
%    \item \textit{Solution:} Ensure that the event loop is running. You can start the event loop using \texttt{asyncio.run()}, \texttt{loop.run\_until\_complete()}, or \texttt{loop.run\_forever()}.
%    \end{itemize}

% 2. \textbf{Blocking Code in the Event Loop}
%    \begin{itemize}
%    \item \textit{Explanation:} If you have blocking code (e.g., a long-running synchronous function) running in the event loop, it can prevent other coroutines from executing.
%    \item \textit{Solution:} Avoid running blocking code in the event loop. Use \texttt{loop.run\_in\_executor()} to offload blocking tasks.
%    \end{itemize}

% 3. \textbf{Incorrect Use of await}
%    \begin{itemize}
%    \item \textit{Explanation:} If you forget to \texttt{await} a coroutine, it won't execute, and the program might appear stuck.
%    \item \textit{Solution:} Always use \texttt{await} when calling a coroutine function.
%    \end{itemize}

% 4. \textbf{Event Loop Blocked by Infinite Loops}
%    \begin{itemize}
%    \item \textit{Explanation:} An infinite loop within a coroutine can prevent the event loop from scheduling other tasks.
%    \item \textit{Solution:} Ensure proper exit conditions and use \texttt{await} within loops.
%    \end{itemize}

% 5. \textbf{Using time.sleep() Instead of asyncio.sleep()}
%    \begin{itemize}
%    \item \textit{Explanation:} \texttt{time.sleep()} is a blocking function that will pause the entire event loop.
%    \item \textit{Solution:} Use \texttt{await asyncio.sleep()} in asynchronous code.
%    \end{itemize}

% \textbf{Code Examples}

% 1. Correct Event Loop Usage:
% \begin{verbatim}
% import asyncio

% async def my_coroutine():
%     print("Starting sleep")
%     await asyncio.sleep(2)
%     print("Finished sleep")

% # Correct way to run the coroutine
% asyncio.run(my_coroutine())
% \end{verbatim}

% 2. Avoiding Blocking Code:
% \begin{verbatim}
% # Bad Example:
% async def blocking_coroutine():
%     time.sleep(10)  # Blocks event loop

% # Good Example:
% async def non_blocking_coroutine():
%     await asyncio.sleep(10)  # Non-blocking
% \end{verbatim}

% 3. Proper await Usage:
% \begin{verbatim}
% # Incorrect:
% async def main():
%     another_coroutine()  # Missing await

% # Correct:
% async def main():
%     await another_coroutine()
% \end{verbatim}

% \textbf{Debugging Tips}
% \begin{itemize}
%     \item Enable Debug Mode:
%     \begin{verbatim}
% asyncio.run(main(), debug=True)
%     \end{verbatim}
%     \item Inspect Tasks:
%     \begin{verbatim}
% tasks = asyncio.all_tasks()
% print(f"Tasks: {tasks}")
%     \end{verbatim}
%     \item Handle Exceptions:
%     \begin{verbatim}
% try:
%     await some_coroutine()
% except Exception as e:
%     print(f"Exception occurred: {e}")
%     \end{verbatim}
% \end{itemize}

% \textbf{Best Practices}
% \begin{itemize}
%     \item Keep the Event Loop Unblocked: Avoid running blocking code
%     \item Use await Appropriately: Always \texttt{await} coroutine functions
%     \item Offload Blocking Tasks: Use \texttt{loop.run\_in\_executor()} for CPU-bound tasks
%     \item Test with Debugging Tools: Utilize asyncio debugging features
% \end{itemize}

% \textbf{Additional Resources}
% \begin{itemize}
%     \item Python asyncio Documentation: \url{https://docs.python.org/3/library/asyncio.html}
%     \item Asynchronous Programming in Python: \url{https://realpython.com/async-io-python/}
%     \item Understanding Asyncio and Event Loops: \url{https://medium.com/swlh/understanding-asyncio-and-event-loops-in-python-af1a57c90e7}
% \end{itemize}

% \end{tiny}
% \end{tcolorbox}

\definecolor{wkblue}{rgb}{0.2, 0.3, 0.6}
\definecolor{meta-color}{rgb}{0.5, 0.5, 0.5}
\definecolor{pinkcolor}{rgb}{1.0, 0.75, 0.8}

\begin{tcolorbox}[
colback=pinkcolor!10!white,
colframe=pinkcolor!100!red,
left=2mm,
right=2mm,
title=\small\centering\textcolor{black}{Complete Guide to await asyncio.sleep() Issues},
breakable=true
]

\section*{Understanding asyncio.sleep()}
When you encounter an issue where \texttt{await asyncio.sleep()} seems to be "stuck" in Python, there are several potential reasons and solutions to consider. Let's delve into this step by step.

First, it's important to understand what \texttt{asyncio.sleep()} does:
\begin{itemize}
\item \texttt{asyncio.sleep()} is a coroutine function that suspends the execution of the coroutine for a given number of seconds
\item During the sleep, other tasks can run, making it useful for simulating delays without blocking the entire program
\item It's commonly used in asynchronous programming to introduce delays or to simulate IO-bound operations
\end{itemize}

\section*{Common Reasons Why await asyncio.sleep() Might Seem Stuck}

\subsection*{1. Event Loop Not Running}
\begin{itemize}
\item \textbf{Explanation:} The asyncio event loop is responsible for managing and scheduling coroutines. If the event loop isn't running, the coroutines won't execute, and \texttt{await asyncio.sleep()} will appear stuck.
\item \textbf{Solution:} Ensure that the event loop is running. You can start the event loop using \texttt{asyncio.run()}, \texttt{loop.run\_until\_complete()}, or \texttt{loop.run\_forever()}.
\end{itemize}

\subsection*{2. Blocking Code in the Event Loop}
\begin{itemize}
\item \textbf{Explanation:} If you have blocking code (e.g., a long-running synchronous function) running in the event loop, it can prevent other coroutines from executing.
\item \textbf{Solution:} Avoid running blocking code in the event loop. Use \texttt{loop.run\_in\_executor()} to offload blocking tasks.
\end{itemize}

\subsection*{3. Incorrect Use of await}
\begin{itemize}
\item \textbf{Explanation:} If you forget to \texttt{await} a coroutine, it won't execute.
\item \textbf{Solution:} Always use \texttt{await} when calling a coroutine function.
\end{itemize}

\subsection*{4. Event Loop Blocked by Infinite Loops}
\begin{itemize}
\item \textbf{Explanation:} An infinite loop within a coroutine can prevent the event loop from scheduling other tasks.
\item \textbf{Solution:} Ensure proper exit conditions and use \texttt{await} within loops.
\end{itemize}

\subsection*{5. Using time.sleep() Instead}
\begin{itemize}
\item \textbf{Explanation:} \texttt{time.sleep()} is a blocking function that will pause the entire event loop.
\item \textbf{Solution:} Use \texttt{await asyncio.sleep()} in asynchronous code.
\end{itemize}

\section*{Step-by-Step Troubleshooting}

\subsection*{1. Verify That the Event Loop Is Running}
Ensure that the event loop is running and your coroutine is scheduled:

\begin{verbatim}
import asyncio

async def my_coroutine():
    print("Starting sleep")
    await asyncio.sleep(2)
    print("Finished sleep")

# Correct way to run the coroutine
asyncio.run(my_coroutine())
\end{verbatim}

For older Python versions (before 3.7):
\begin{verbatim}
loop = asyncio.get_event_loop()
loop.run_until_complete(my_coroutine())
\end{verbatim}

\subsection*{2. Check for Blocking Code}
Bad Example:
\begin{verbatim}
import asyncio
import time

async def blocking_coroutine():
    print("Starting blocking operation")
    time.sleep(10)  # Blocks the event loop
    print("Finished blocking operation")

asyncio.run(blocking_coroutine())
\end{verbatim}

Good Example:
\begin{verbatim}
import asyncio

async def non_blocking_coroutine():
    print("Starting sleep")
    await asyncio.sleep(10)
    print("Finished sleep")

asyncio.run(non_blocking_coroutine())
\end{verbatim}

\subsection*{3. Ensure Proper Use of await}
Incorrect:
\begin{verbatim}
import asyncio

async def another_coroutine():
    print("This coroutine won't be awaited")

async def main():
    another_coroutine()  # Missing await
    print("Main coroutine continues")

asyncio.run(main())
\end{verbatim}

Correct:
\begin{verbatim}
import asyncio

async def another_coroutine():
    print("This coroutine is awaited")

async def main():
    await another_coroutine()  # Properly awaited
    print("Main coroutine continues")

asyncio.run(main())
\end{verbatim}

\subsection*{4. Avoid Infinite Loops}
Bad Example:
\begin{verbatim}
import asyncio

async def infinite_loop_coroutine():
    while True:
        print("Looping...")
        # Missing await inside the loop
        # await asyncio.sleep(1)

asyncio.run(infinite_loop_coroutine())
\end{verbatim}

Good Example:
\begin{verbatim}
import asyncio

async def controlled_loop_coroutine():
    while True:
        print("Looping...")
        await asyncio.sleep(1)  # Allows switching tasks

asyncio.run(controlled_loop_coroutine())
\end{verbatim}

\subsection*{5. Use asyncio.run\_in\_executor() for Blocking Tasks}
\begin{verbatim}
import asyncio
import time

def blocking_function():
    time.sleep(10)
    return "Blocking function completed"

async def main():
    loop = asyncio.get_running_loop()
    result = await loop.run_in_executor(None, blocking_function)
    print(result)

asyncio.run(main())
\end{verbatim}

\section*{Debugging Tips}

Enable Debug Mode:
\begin{verbatim}
asyncio.run(main(), debug=True)
\end{verbatim}

Inspect Tasks:
\begin{verbatim}
tasks = asyncio.all_tasks()
print(f"Tasks: {tasks}")
\end{verbatim}

Exception Handling:
\begin{verbatim}
try:
    await some_coroutine()
except Exception as e:
    print(f"Exception occurred: {e}")
\end{verbatim}

\section*{Example of a Common Mistake}
Mixing synchronous and asynchronous code:
\begin{verbatim}
import asyncio

async def async_function():
    print("Async function started")
    await asyncio.sleep(5)
    print("Async function finished")

def sync_function():
    print("Sync function started")
    time.sleep(10)
    print("Sync function finished")

async def main():
    task = asyncio.create_task(async_function())
    sync_function()  # Blocks for 10 seconds
    await task

asyncio.run(main())
\end{verbatim}

Output:
\begin{verbatim}
Async function started
Sync function started
# 10 seconds later
Sync function finished
# 5 seconds later
Async function finished
\end{verbatim}

\section*{Best Practices}
\begin{itemize}
\item Keep the Event Loop Unblocked: Avoid running blocking code
\item Use await Appropriately: Always await coroutine functions
\item Offload Blocking Tasks: Use loop.run\_in\_executor()
\item Test with Debugging Tools: Utilize asyncio debugging features
\end{itemize}

\section*{Conclusion}
If \texttt{await asyncio.sleep()} seems stuck, it's likely due to the event loop being blocked or not running properly. By ensuring the event loop is active, avoiding blocking code, and using \texttt{await} correctly, you can resolve the issue and ensure smooth asynchronous execution in your Python programs.

\section*{Additional Resources}
\begin{itemize}
\item Python asyncio Documentation: \url{https://docs.python.org/3/library/asyncio.html}
\item Asynchronous Programming in Python: \url{https://realpython.com/async-io-python/}
\item Understanding Asyncio and Event Loops: \url{https://medium.com/swlh/understanding-asyncio-and-event-loops-in-python-af1a57c90e7}
\end{itemize}

\end{tcolorbox}
